Deflecting the Value Compass: Interacting with Large Language Models Temporarily Shifts Human Value Priorities Toward Personal Focus

Large language models increasingly support decisions where values are in tension, yet little is known about whether interacting with them changes which values users prioritize. In a preregistered study, 200 U.S. adults interacted with ChatGPT, Claude, or Gemini as a thinking partner or read fixed AI-generated considerations. The prompt asked LLMs to support reasoning without recommending a decision and named no values. Participants advised people facing real dilemmas and completed parallel PVQ-RR forms before, immediately after, and one task later. Each LLM condition temporarily shifted value priorities toward personal focus relative to the control (d=0.37-0.51), primarily through increased Self-Enhancement. Participants' advice retained words and meaning from their exchanges. Thus, a brief LLM interaction that neither targets values nor seeks to persuade can reorient values active during judgment without detectable convergence in value directions or advice.

==> fig/tokens.tex <==
% GENERATED by `python -m figstyle emit-tex` -- DO NOT EDIT.
% Edit figstyle/tokens.py and regenerate. `make check` fails if this
% file's digest no longer matches the tokens it was generated from.
% figstyle-tokens-sha256: 035fd656685245552957e1d06d16cd2e07973652ad56fec1ae98cfe678f8f376

\RequirePackage{xcolor}
\RequirePackage{graphicx}

% --- arm marks: a hue means a live model wrote the text, ink means it did not
\definecolor{figBaseline}{HTML}{3F3F46}
\definecolor{figChatGPT}{HTML}{0B3CCB}
\definecolor{figClaude}{HTML}{C14624}
\definecolor{figGemini}{HTML}{B0882F}

% --- arm text steps: the same hues darkened to clear 4.5:1 on white
\definecolor{figBaselineText}{HTML}{27272A}
\definecolor{figChatGPTText}{HTML}{042CAC}
\definecolor{figClaudeText}{HTML}{74240C}
\definecolor{figGeminiText}{HTML}{533F11}

% --- neutral ramp (shadcn zinc)
\definecolor{figZinc50}{HTML}{FAFAFA}
\definecolor{figZinc100}{HTML}{F4F4F5}
\definecolor{figZinc200}{HTML}{E4E4E7}
\definecolor{figZinc300}{HTML}{D4D4D8}
\definecolor{figZinc400}{HTML}{A1A1AA}
\definecolor{figZinc500}{HTML}{71717A}
\definecolor{figZinc600}{HTML}{52525B}
\definecolor{figZinc700}{HTML}{3F3F46}
\definecolor{figZinc800}{HTML}{27272A}
\definecolor{figZinc900}{HTML}{18181B}
\definecolor{figZinc950}{HTML}{09090B}

% --- semantic roles
\definecolor{figPage}{HTML}{FFFFFF}
\definecolor{figSurface}{HTML}{FFFFFF}
\definecolor{figBand}{HTML}{F4F4F5}
\definecolor{figBandAlt}{HTML}{FAFAFA}
\definecolor{figBorder}{HTML}{E4E4E7}
\definecolor{figGrid}{HTML}{E4E4E7}
\definecolor{figRule}{HTML}{D4D4D8}
\definecolor{figNS}{HTML}{A1A1AA}
\definecolor{figMutedFg}{HTML}{71717A}
\definecolor{figSecondaryFg}{HTML}{52525B}
\definecolor{figFg}{HTML}{18181B}

% --- prose macros, so an arm named in the text wears its figure colour
% \arm{Claude} -> the word, in Claude's text step
\newcommand{\arm}[1]{{\color{fig#1Text}#1}}
% \armtext{Gemini}{whatever} -> arbitrary text in an arm's colour
\newcommand{\armtext}[2]{{\color{fig#1Text}#2}}
% \armswatch{ChatGPT} -> an inline legend square in the MARK colour
\newcommand{\armswatch}[1]{\textcolor{fig#1}{\rule[0.15ex]{1.1ex}{1.1ex}}}

% --- the only sanctioned figure inclusion.
% Figures are generated at exactly 428bp against acmart
% manuscript's 430.005 TeX pt \textwidth, so \figincl{name} places one at
% its natural size with 0.4 pt of slack and no key needed.
%
% The optional argument goes straight to \includegraphics, so
% \figincl[width=0.75\textwidth]{name} and \figincl[scale=0.75]{name} both
% work. Scaling costs type: at 0.75 a 6.2 pt label lands at 4.65 pt,
% under the 6.2 pt floor. Worth knowing rather than worth forbidding --
% a screenshot has no tick labels to shrink.
\newcommand{\figincl}[2][]{\includegraphics[#1]{fig/#2}}

